MultiViz: Towards Visualizing and Understanding Multimodal Models

The promise of multimodal models for real-world applications has inspired research in visualizing and understanding their internal mechanics with the end goal of empowering stakeholders to visualize model behavior, perform model debugging, and promote trust in machine learning models. However, modern multimodal models are typically black-box neural networks, which makes it challenging to understand their internal mechanics. How can we visualize the internal modeling of multimodal interactions in these models? Our paper aims to fill this gap by proposing MultiViz, a method for analyzing the behavior of multimodal models by scaffolding the problem of interpretability into 4 stages: (1) unimodal importance: how each modality contributes towards downstream modeling and prediction, (2) cross-modal interactions: how different modalities relate with each other, (3) multimodal representations: how unimodal and cross-modal interactions are represented in decision-level features, and (4) multimodal prediction: how decision-level features are composed to make a prediction. MultiViz is designed to operate on diverse modalities, models, tasks, and research areas. Through experiments on 8 trained models across 6 real-world tasks, we show that the complementary stages in MultiViz together enable users to (1) simulate model predictions, (2) assign interpretable concepts to features, (3) perform error analysis on model misclassifications, and (4) use insights from error analysis to debug models. MultiViz is publicly available, will be regularly updated with new interpretation tools and metrics, and welcomes inputs from the community.

==> figures/methods.tex <==
\begin{figure}[tbp]
\centering
\vspace{-6mm}
\includegraphics[width=0.7\linewidth]{figures/methods_fig.pdf}
\vspace{0mm}
\caption{\names\ is a comprehensive analysis benchmark encompassing a set of fine-grained analysis tools across multiple stages: (1) unimodal importance, (2) cross-modal interactions, (3) multimodal representations, and (4) multimodal prediction.}
\label{fig:methods}
\vspace{-4mm}
\end{figure}

==> figures/representation.tex <==
\begin{figure}[tbp]
\centering
\vspace{-6mm}
\includegraphics[width=0.7\linewidth]{figures/representation_fig.pdf}
\vspace{0mm}
\caption{We visualize multimodal representations through local and global analysis. Given an input datapoint, \textbf{local analysis} visualizes the unimodal and cross-modal interactions that activate a feature. \textbf{Global analysis} informs the user of similar datapoints that also maximally activate that feature, and is especially useful in assigning human-interpretable concepts to features by looking at similarly activated input regions across datapoints (e.g., the concept of color in this case).}
\label{fig:representation}
\vspace{-4mm}
\end{figure}
